AABAC -- Automated Attribute Based Access Control for Genomics Data

The COVID-19 crisis has demonstrated the potential of cutting-edge genomics research. However, privacy of these sensitive pieces of information is an area of significant concern for genomics researchers. The current security models makes it difficult to create flexible and automated data sharing frameworks. These models also increases the complexity of adding or revoking access without contacting the data publisher. In this work, we investigate an automated attribute-based access control (AABAC) model for genomics data over Named Data Networking (NDN). AABAC secures the data itself rather than the storage location or transmission channel, provides automated data invalidation, and automates key retrieval and data validation while maintaining the ability to control access. We show that AABC when combined with NDN provide a secure and flexible combination for work with genomics research.

==> 3-motivation.tex <==
\section{Motivations}

Currently, to access IRB-secured data, an organization must go through an often lengthy bureaucratic process that includes everyone who will be accessing the data. The long wait times mean that users, including graduate research assistants, sometimes change before even being approved with the current process. This requires more paperwork to amend access. Similar paperwork is also needed whenever someone leaves the project. The current solution also has all the data protection mechanisms controlled and distributed by IRB. However, the IRB often lacks the cybersecurity expertise to fully evaluate and appreciate the potential vulnerabilities inherent in the current approaches. The primary function of the IRB is to evaluate the risk, rights, and welfare of human participants relative to the benefits of participating in the research. The final responsibility for ensuring the safety, integrity, and access to the data is delegated to the primary investigator\cite{amdur2010institutional}.

The IRB requirements also have strict data retention and access requirements that still leave many security holes and bypasses vulnerable to a system administrator or someone with physical access. One of the problems is that, currently, once the secure data arrives at the secure server, Linux access controls are used to maintain data security. This access control model also means that the information is no longer individually encrypted once on the secure server.

Our proposed solution would mitigate some of these problems, along with a more efficient distribution system, by allowing more effortless flexibility to change who is authorized and better secure the data. For our design, we utilize two attributed authorities (henceforth referred to as "ledgers"). The problem of flexible access control is solved using a two-tier ledger access system we designed. The first ledger is a remote one possibly controlled by IRB and gives broad attributes. The other ledger would be local and then provide the users with permission to access the data.

For example, such a schema might encrypt data with the following attributes:
\begin{verbatim}
    the PI and 
    PI's selected graduate students and
    PI's selected collaborators.
\end{verbatim} 

The PI then can add or remove graduate students and collaborators as needed. The security and key distribution would then be solved using CP-ABE (attribute-based encryption). CP-ABE encryption allows the data to be encrypted at the source and then have the access model changed in the future. A name-based network can distribute the keys and data. With this scheme, it is unnecessary to decide who will access the data when it is published or made available. 


==> 5.2-scenarios-full.tex <==
\section{Possible Real-World Scenarios}
\todo[inline]{Just pick 2 scenarios and the table. Also update the scenarios}
%\todo[inline]{For each of these - show the name of the content and what the key name will look like. Show what are the benefits of this model.}
% Not exactly sure what you mean with the key name, I added in previous section now the use of the attributes for the keys thou. 

Having explored the motivation and design for the proposed system in this paper, we aim to demonstrate the system's effectiveness with real-world situations. The distinct scenarios will be primarily based on a hypothetical access framework. The PI is a faculty working for department A. Being a faculty, the PI also has a graduate assistant B assisting with project X. These scenarios are demonstrated in Table \ref{tab:attributeTable} outlining attributes and attribute policies. 
    
    
    %PI requests for the      required resources and allows graduate assistant     B to view and update PI's resources. Similarly,      PI allows collaborator at university C who in-turn allows graduate assistant D to view and update the resource's data.
    
\subsection{Scenario/Use Case 1}
In the first use case, there is only one institution, one department, one PI, and multiple students working under the PI with the title graduate assistant. One or more of the graduate assistants are involved in the genomics project. The PI grants access only to those assistants involved in the genomics project. Assistants who are not on the project but share the same title as the PI's assistants will not have access to the resources. By using this model, students are assigned to the project easily but securely. While not showing many advantages over PKI, more complex scenarios would.


    \subsubsection{Attributes}
Project, Principal Investigator, Role

    \subsubsection{Requested Content Name}
\name{Genome1/SRA/9605/9606/RNA-Seq/1}

    \subsubsection{User receives content and requests decryption Key Name from Local Ledger}
\name{/Genome1/SRA/9605/9606/RNA-Seq1/DecryptionKey/Attributes/Name=John Smith/Project=Genome1/Role=Graduate Assistant}

    \subsubsection{Access Control Rule and Trust Schema}
    Return symmetric key decryption key - [(Project = Genome1) and (PI = John Smith) and (Role = Graduate Assistant)]

\subsubsection{Example}
    \begin{itemize}
        \item Student 1 - [Project = Genome1; PI = John Smith; Role = Graduate Assistant] - Receives personal decryption key
        \item Student 2 - [Project = Biology1; PI = John Smith; Role = Graduate Assistant] - Does not receive decryption key
    \end{itemize}


\subsection{Scenario/Use Case 2}
As the first use case, there is only one institution, but more than one department as the PI has multiple collaborators from the same or different department. The PI collaborates with a faculty of department A and another from department C. Under such circumstances, a faculty of department D or E will not be able to view or update the project resources. This scenario shows the ability to easily give members of different departments, who may only have access to portions of the data, without requiring a unique public key encryption of every symmetric key that would create scaling issues and unnecessary management work. Instead, this design allows a symmetric key for each segment to be encrypted once with a restrictive policy rather than for each user.

    \subsubsection{Attributes}
    Principal Investigator, Department, Role
    
    \subsubsection{Requested Content Name}
    \name{Genome1/SRA/9605/9606/RNA-Seq/1}

    \subsubsection{User receives content and requests decryption Key Name from Local Ledger}
    \name{/Genome1/SRA/9605/9606/RNA-Seq1/DecryptionKey/Attributes/Name=John Smith/Department=Computer Science/Role=Graduate Assistant}

    \subsubsection{Access Control Rule and Trust Schema}
    Return symmetric key decryption key - [(PI = John Smith) and (Department = Biology or Department = Computer Science) and (Role = Faculty)]
    
    \subsubsection{Example}
    \begin{itemize}
        \item Faculty 1 (allowed) - [PI = John Smith; Department = Biology; Role = Faculty]
        \item Faculty 2 (not allowed) - [PI = John Smith; Department = Physics; Role = Faculty]
    \end{itemize}
 
\subsection{Scenario/Use Case 3}
There may be two departments from two different institutions working collaboratively on a single project. The project may include two PIs and multiple graduate assistants working in collaborations. Based on this scenario, the attribute for providing access to the project-related resources would potentially rely on the university's name, the department, and the project. The graduate assistants must be employed under the PIs and assigned to the specific project to access the resources. Anyone outside this group will not be able to update or view the data. With more complex key requirements like multiple institutions, this model is demonstrated to handle the problem with little extra key management due to the policy being created once. This model also has the data and key distribution from NDN and does not require each institution to handle the many encrypted keys, and enables each institution to download any required samples securely from NDN easily.

    \subsubsection{Attributes}
    Project, Principal Investigator, University, Department, Role
    
    \subsubsection{Requested Content Name}
    \name{Genome1/SRA/9605/9606/RNA-Seq/1}

    \subsubsection{User receives content and requests decryption Key Name from Local Ledger}
    \name{/Genome1/SRA/9605/9606/RNA-Seq1/DecryptionKey/Attributes/Name=John Smith/Project=Genome1/University=MIT/Department=Biology/Role=Graduate Assistant}

    \subsubsection{Access Control Rule and Trust Schema}
    Return symmetric key decryption key - [(Project = Genome1) and (((PI = John Smith) and (University = MIT) and (Department = Biology or Department = Computer Science) and (Role = Graduate Assistant)) or ((PI = Jack Robinson) and (University = UCLA) and (Department = Biology or Department = Computer Science) and (Role = Graduate Assistant)))]
    
    \subsubsection{Example}
    \begin{itemize}
        \item Student 1 (allowed) - [Project = Genome1; PI = John Smith; University = MIT; Department = Biology; Role = Graduate Assistant]
        \item Student 2 (not allowed) - [Project = Genome1; PI = John Smith; University = UCLA; Department = Biology; Role = Graduate Assistant]
    \end{itemize}
 

\subsection{Scenario/Use Case 4}
Data science, machine learning, and artificial intelligence-related research work have become so interdisciplinary that a faculty from the same or a different department at an institution may request access to the genomics resources for teaching or other academic research-based purposes. In this situation, the requester's attributes will need to be added to the local ledger so that the researcher can extract the necessary information. Here, the related work may be an extension of the target project, e.g. project X. Some additional attributes may be required to limit the access of the external researcher to only those required resources. The NDN distribution would also verify what they can access based on the researcher's policies in their keys.

    \subsubsection{Attributes}
Main Project, Sub Project, Principal Investigator, Department, Role

    \subsubsection{Requested Content Name}
    \name{Genome1/SRA/9605/9606/RNA-Seq/1}

    \subsubsection{User receives content and requests decryption Key Name from Local Ledger}
    \name{/Genome1/SRA/9605/9606/RNA-Seq1/DecryptionKey/Attributes/Name=John Smith/Project=Genome1/SubProject=Computation1/Department=Computer Science/Role=Faculty}

    \subsubsection{Access Control Rule and Trust Schema}
    Return symmetric key decryption key - [(Main Project = Genome1) and (Sub Project = Computation1 or Sub Project = Animalia1) and (PI = John Smith) and (Department = Biology or Department = Computer Science) and (Role = Faculty)]

    \subsubsection{Example}
    \begin{itemize}
        \item Faculty 1 (allowed) - [Main Project = Genome1; Sub Project = Computation1; PI = John Smith; Department = Computer Science; Role = Faculty]
        \item Faculty 2 (not allowed) - [Main Project = Genome1; Sub Project = Physics1; PI = John Smith; Department = Physics; Role = Faculty]
    \end{itemize}

\subsection{Scenario/Use Case 5}
One of the graduate assistants submits his/her dissertation of the work performed for the project and graduates from institution A. The assistant's credentials will be removed from project X's list of collaborators, which will revoke all access rights for the recent graduate. 

    \subsubsection{Attributes}
    Project, Principal Investigator, Role, Date
    
    \subsubsection{Requested Content Name}
    \name{Genome1/SRA/9605/9606/RNA-Seq/1}

    \subsubsection{User receives content and requests decryption Key Name from Local Ledger}
    \name{/Genome1/SRA/9605/9606/RNA-Seq1/DecryptionKey/Attributes/Name=John Smith/Project=Genome1/Role=Graduate Assistant/Date=04/21/2021/Valid=True}

    \subsubsection{Access Control Rule and Trust Schema}
    Return symmetric key decryption key - [(Project = Genome1) and (PI = John Smith) and (Role = Graduate Assistant) and (Date <= 05/01/2021) and IS\_VALID]
    
    \subsubsection{Example}
    \begin{itemize}
        \item Student 1 (allowed) - [Project = Genome1; PI = John Smith; Role = Graduate Assistant; Date = (Current Date = 04/21/2021), IS\_VALID=True]
        \item Student 2 (not allowed) - [Project = Genome1; PI = John Smith; Role = Graduate Assistant; Date = (Current Date = 05/02/2021), IS\_VALID = False]
    \end{itemize}

As discussed earlier, when IS\_VALID is set to False, the student will no longer be able to decrypt the data. However, they will be able to utilize any previously decrypted data still. Simple operational remediation is to revoke the filesystem access of the student.

\begin{table*}[ht!]
\caption{This table lists the attributes and attribute policies used for each of the seven scenarios tested along with the result.}
\begin{center}

    \begin{tabular}{|p{0.9cm}|p{7.5cm}|p{7.5cm}|}
    \hline
    Scenario No. & Attributes Used & Attribute Policy\\
    \hline
    1. & Genome1, Genome2, John Smith, and Graduate Assistant & Genome1 and John Smith and Graduate Assistant\\
    \hline
    2. & John Smith, Biology, Physics, and Faculty & John Smith and (Biology or Computer Science) and Faculty\\
    \hline
    3. & Genome1, John Smith, TN Tech, Clemson, Biology, and Graduate Assistant & Genome1 and ((John Smith and TN Tech and (Biology or Computer Science) and Graduate Assistant) or (Jack Robinson and Clemson and (Biology or Computer Science) and Graduate Assistant))\\
    \hline
    4. & Genome1, Computation1, Physics1, John Smith, Computer Science, Physics, and Faculty & Genome1 and (Computation1 or Animalia1) and John Smith and (Biology or Computer Science) and Faculty\\
    \hline
    5. & Genome1, John Smith, Graduate Assistant, Current Date (04/21/2021), and Current Date (05/02/2021) & Genome1 and John Smith and Graduate Assistant and Current Date < 05/01/2021\\
    \hline
    \end{tabular}
    \vspace{-2em}
    \label{tab:attributeTable}
\end{center}
\end{table*}
 
